Understanding High-Order Network Structure using Permissible Walks on Attributed Hypergraphs

Hypergraphs have been a recent focus of study in mathematical data science as a tool to understand complex networks with high-order connections. One question of particular relevance is how to leverage information carried in hypergraph attributions when doing walk-based techniques. In this work, we focus on a new generalization of a walk in a network that recovers previous approaches and allows for a description of permissible walks in hypergraphs. Permissible walk graphs are constructed by intersecting the attributed $s$-line graph of a hypergraph with a relation respecting graph. The attribution of the hypergraph's line graph commonly carries over information from categorical and temporal attributions of the original hypergraph. To demonstrate this approach on a temporally attributed example, we apply our framework to a Reddit data set composed of hyperedges as threads and authors as nodes where post times are tracked.

==> sections/method_old.tex <==
%!TEX root = ..\main.tex
%-------------------------------------------------
%*************************************************


\evg{Some general comments:}

\evg{
\begin{itemize}
    \item some notions are used without definition (abstract simplicial complex, extension of a line graph); some notion are defined after they are used (e.g. proposition 5 happens before definition 6)
    \item if something is a function (in a mathematical sense), the domain and range should be specified/clear (and the symbols that denote domain and range should be defined )
    \item the definition that i get from wiki for the term relation: for a set $X$, relation is a subset of $X\times X$. Thus, attributes need to be at least a set
    \item from what i see, one of the goals of section 1 was to get to the definition of the permissible s-line graph. So why not get to it as soon as one can and only after have all the discussion about the possible attributes and how one can go from one set of attributes to another.
\end{itemize}
}

\section{Background and Method} \label{sec:method}

In this section, we present our methodology for constructing a permissible walk graph from an attributed hypergraph. The general procedure is {exemplified} in Fig.~\ref{fig:pipeline_permissible_walks}. We provide both the method and the necessary background for understanding the construction of the permissible walk graph. To illustrate the steps involved, we also include a toy example throughout this section. While our example is attributed with temporal and categorical information, any attribute could be used as long as a relation can be assigned based on the attributes.

\begin{figure}[h!] 
    \centering
    \includegraphics[width=.7\textwidth]{figures/PW_graph_pipeline.pdf}%
    \caption{The pipeline for generating the permissible walk graph starting with an attributed hypergraph (described in Section~\ref{ssec:attributed_HG}), which is used to construct the attributed $s$-line graph using an attribute transferring function (see Section~\ref{ssec:attributed_line_graph}). The permissible walk graph is then constructed as an attribute respecting subgraph of the $s$-line graph (see Section~\ref{ssec:permissible_walk_graph}).}
    \label{fig:pipeline_permissible_walks}
\end{figure}

We start with our definition of an attributed hypergraph in Section~\ref{ssec:attributed_HG}. Next, in Section~\ref{ssec:attributed_line_graph} we overview how to construct the attributed line graph from the attributed hypergraph by transferring attributes.
Lastly, in section~\ref{ssec:permissible_walk_graph} we show how the permissible walk graph is constructed from the attributed line graph which is demonstrated using our toy example.

\subsection{Attributed Hypergraphs} \label{ssec:attributed_HG}

\begin{defn}
Let $H = \tup{ V, E, \phi, \epsilon, \gamma }$ be an {\bf attributed hypergraph}, where
$V$ is a finite, non-empty set of {\bf vertices} with $|V|=n$;
$E$ is a finite, non-empty set of {\bf edges} or {\bf hyperedges} with $|E|=m$; 
$\func{\phi}{V}{X}$ is the {\bf vertex attribute function} to a set of vertex attributes $X$;    
$\func{\epsilon}{E}{Y}$ is the {\bf edge attribute function} to a set of edge attributes $Y$; and     $\func{\gamma}{V \times E}{Z \sqcup \{ \emptyset \}}$ is the {\bf incidence attribute function} to a set of incidence attributes $Z$.
\end{defn}


The incidence attribute function $\gamma$ identifies a binary relation $R \sub V \times E$ where $\tup{v,e} \in R \iff \gamma(v,e) \neq \emptyset$. 
$\gamma$ also identifies a  Boolean characteristic function  $\func{I}{V \times E}{\{0,1\}}$ where
				\[ I(v,e) = \halffunc{
		1,	& \gamma(v,e) \neq \emptyset	\\
									0,	& \gamma(v,e) = \emptyset	
			}.	\]
By abuse of notation we also represent $I$ as the incidence matrix $I_{n \times m}$ where simply $I[v,e] = I(v,e)$.

We call the vertices $v \in V$ and edges $e \in E$ generically {\bf objects}.
The images of the objects in the relation $R$ establish two ``marginal'' functions $\func{R_V}{V}{2^E}$ and $\func{R_E}{E}{2^V}$ taking vertices to sets of edges and edges to sets of vertices respectively:
			 \[ R_V(v) = \{ e \in E \st \tup{v,e} \in R \},	\qquad
			 	R_E(e) = \{ v \in V \st \tup{v,e} \in R \}.	\]
    This construction establishes a base multihypergraph, also denoted $H = \tup{V,E}$, in that we can identify the edges  $e \in E$ as subsets $R_E(e) \sub V$ of vertices, where $v \in e \iff \gamma(v,e) \neq \emptyset$. Note that $E$ is not a set of subsets of $V$ (is not a subset of $2^V$), but rather an indexed family of subsets of $V$: this is an interpretation of $E$ as a multiset possibly containing duplicate edges.     Let the size $N \define \max_{e \in E} |R_E(e)|$ of the largest edge of the hypergraph be called its {dimension}.

We say that $H$ is the {\bf primal} pointing, because we also have
 the {\bf dual} hypergraph $H^* = \tup{ E, V, \epsilon, \phi, \gamma^* }$, with now vertices $v \in V$ as sets $R_V(v) \sub E$ and incidence matrix $I^T_{m \times n}$ with $\func{\gamma^*}{E \times V}{Z \sqcup \emptyset }$ and $\gamma^*(e,v) = \gamma(v,e)$. The dual hypergraph  has dimension $M \define \max_{v \in V} |R_V(v)|$.
 

While any attribute type could be applied to the hypergraph, our method requires that a relation $R$ can be defined on the set of attributes to form a permissible walk graph (e.g., $R \subseteq Y \times Y$ for a relation between edge attributes).  
Some common attribute types that would allow for a relation to be defined are as follows: 
\begin{itemize}
    \item {\bf {Logical Attributes}}: For logical attributes $\phi$, $\epsilon$, and $\gamma$ can take values in $\{0,1\}$. Relations can then be defined based on logical expressions (e.g., and/or).
    \item  {\bf Semantic Type Hierarchy Attributes}: $\gamma \in {\cal L}$ semantic type hierarchy, where $\mathcal{L}$ is a hierarchical data structure, which has an underlying poset. The relation is then implied by the hierarchy.
    \item  {\bf Set Attributes}: For the set attribute type, consider $\phi$, $\epsilon$, and $\gamma$ taking values in a set without any additional structure applied.
We can define a relation on these sets using an intersection criteria such that they are related if they intersect by at least $t$ nodes. 
We consider this attribute type in our toy example with sets attributed on each incidence as shown in Fig.~\ref{fig:topic_attributes}.

    \item  {\bf Temporal Attributes}: For temporal attributes, the functions $\phi$, $\epsilon$, and $\gamma$ take assign intervals. a relation between intervals can be defined in many ways including weak, strong, or inclusion orders~\cite{joslyn}. An example of interval attributes on the edges as $\epsilon: E \to Y$ is shown in Fig.~\ref{fig:interval_attributes} of our toy example with intervals attributed to the edges.
\end{itemize}

\paragraph{Example}
For our toy example attributed hypergraph (see Fig.~\ref{fig:meeting_HG}) we set interval attributes on the edges as shown in Fig.~\ref{fig:interval_attributes} and topic attributes on the incidences as shown in Fig.~\ref{fig:topic_attributes}. This attributed hypergraph is meant to model four meetings $[M_1 \ldots, M_4]$ that occurred between six people $[P_1, \ldots, P_6]$ with a total of six topics discussed $[A, B, \ldots, F]$. The incidence attributes $Z$ of topics in Fig.~\ref{fig:topic_attributes} represent which topics were discussed by which people in each meeting (e.g., person $P_4$ discussed topics $(A, B)$ in meeting $M_1$) and the interval attributes in Fig.~\ref{fig:interval_attributes} describe when the meeting occurred (e.g., $M_1$ occurred from time 0 to 1).

\begin{figure}[h!] 
    \centering
    \begin{subfigure}[b]{.3\textwidth}
        \centering
        \includegraphics[width=.99\textwidth]{figures/meeting_HG.png}
        \vspace*{-10mm}
        \caption{Meeting hypergraph.}
        \label{fig:meeting_HG}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.3\textwidth}
        \centering
        \includegraphics[width=.99\textwidth]{figures/meeting_intervals.png}%
        \caption{Time interval edge attributes.}
        \label{fig:interval_attributes}
    \end{subfigure}
    \hfill
    \begin{subtable}[b]{.35\textwidth}
        \centering
        \begin{tabular}{ccccc}
                                   & $M_1$       & $M_2$       & $M_3$       & $M_4$       \\ \cline{2-5} 
        \multicolumn{1}{c|}{$P_1$} & $\emptyset$ & $\emptyset$ & $\emptyset$ & $\{C\}$       \\
        \multicolumn{1}{c|}{$P_2$} & $\emptyset$ & $\emptyset$ & $\{C, D\}$    & $\{C\}$       \\
        \multicolumn{1}{c|}{$P_3$} & $\emptyset$ & $\emptyset$ & $\{B, C\}$ & $\{C\}$       \\
        \multicolumn{1}{c|}{$P_4$} & $\{A, B\}$    & $\emptyset$ & $\{D\}$       & $\emptyset$ \\
        \multicolumn{1}{c|}{$P_5$} & $\{A, C\}$    & $\{E, F\}$    & $\emptyset$ & $\emptyset$ \\
        \multicolumn{1}{c|}{$P_6$} & $\emptyset$ & $\{F\}$       & $\emptyset$ & $\emptyset$
        \end{tabular}
        \vspace*{6mm}
        \caption{Topic incidence attributes.}
        \label{fig:topic_attributes}
    \end{subtable}
    \caption{Attributed hypergraph of meetings with meeting time intervals as edge attributes and topics as incidence attributes.}
    \label{fig:attributed_meeting_HG_example}
\end{figure}

While relations can be defined on edge, incidence, or vertex attributes, it may be more useful to associate the attributes from one attribute location to another, which we refer to as an attribute association function. The three types of association functions we consider are vertex marginalization $\func{f_X}{Z^2}{X}$, edge marginalization $\func{f_Y}{Z^2}{Y}$, and extensions $\func{f_Z}{X \times Y}{Z}$. 
Both marginalization functions apply a function to represent the attributes in the incidences to either the edges or vertices.
In our toy example we demonstrate an edge marginalization function $f_Y$ as the union of topic sets on the incidences resulting in $\epsilon(M_1) = \{A, B, C\}$, $\epsilon(M_2) = \{E, F\}$, $\epsilon(M_3) = \{B, C, D\}$, and $\epsilon(M_4) = \{C\}$. We apply this marginalization since, for example, it may be more useful to know the set of topics discussed in a meeting instead of which topics were discussed by which people.
We also have another example of an edge marginalization function in the results of Section~\ref{sec:results} for temporal attributes by taking the convex hull of intervals attributed to incidences.
While the marginalization functions condense incidence attributes to the edges or vertices, the extension function brings edge and vertex attributes to the incidences. For example, we could do an extension of the intervals as edge attributes to the incidences by setting an incidence attribute for each vertex in a hyperedge as the hyperedge's attribute. For example, $P_4$ and $P_5$ in meeting $M_1$ could have extended incidence attributes of the interval $[0,1]$ since meeting $M_1$ has the interval attribute $[0,1]$.


\subsection{Attributed Line Graph} \label{ssec:attributed_line_graph}

To introduce the attributed $s$-line graph we first begin by describing the line graph of a hypergraph.  To start, consider the {\bf $k$-sections} of an attributed HG as the Abstract Simplicial Complex (ASC) of dimension $k$ implied by its sub-hypergraphs also of dimension $k$. Formally,
\begin{defn}[$k$-Sections]
	Given an attributed hypergraph $H$, then define its $k$-th section $H_k$, for $k \le N$, as the ASC
	  \[ H_k = \bigcup_{e \in E} \{ G \sub R_E(e) \st |G| \le k \}.	\]
	  It's $k$-th dual section $H_k^*$ for $k \le M$ is then 
	  \[ H^*_k = \bigcup_{v \in V} \{ G \sub R_V(v) \st |G| \le k \}.	\]
\end{defn}
A special case of the $k$-sections are for dimension $k=2$.
\begin{defn}
	  We call $H_2$ the {\bf clique expansion} or {\bf underlying graph}, and we call $H^*_2$ the {\bf line graph}.%
	  \footnote{Formally, $H_2$ and $H^*_2$ are not graphs, given that they're closed by subset to include all singletons, and thus not 2-uniform. But as defined these are bijective to those graphs.}
\end{defn}

A generalization of the line graph $H_2$ is the $s$-line graph~\cite{aksoy2020hypernetwork}.
\begin{defn}
The {\bf $s$-line graph} $L_s(H) = \tup{E, V} \subseteq H^*_2$  of a hypergraph $H\tup{V,E}$, which has the hyperedge set $E$ of the original hypergraph $H$ as the vertex set of $L_s(H)$ and edge set $D\subseteq E\times E$ with edge $(e_i, e_j) \in D$ if hyperedges $|e_i \cap e_j| \geq s$ with $e_i, e_j\in E$.
\end{defn}
From the $s$-line graph we can set the attributes from the attributed hypergraph to the $s$-line graph as the attributed $s$-line graph.
\begin{defn}
The \textbf{attributed $s$-line graph} $\mathcal{L}_s(H) = (E,D,\tau,\zeta)$ is the $s$-line graph $L_s(H)=(E,K)$ along with $\tau:E\to A$, the attributes of the vertices of $L(H)$, and $\zeta: D \to B$, the attributes of the edges of $L(H)$ , where $A$ and $B$ are the vertex and edge attributes of $\mathcal{L}_s(H)$.
\end{defn} 

Given an attributed hypergraph $H = (V, E, \phi, \epsilon, \gamma)$ and attributed $s$-line graph $G = \mathcal{L}_s(H) = (E, D, \tau, \zeta)$, we need to a method of transferring the attributes $X, Y, Z$ to the attributed line graph. To do this we define an attribute transfer functions to transfer attributes to the vertices and edges of $\mathcal{L}_s$.

\adm{The induced attribute function where tau is the same as epsilon, but slightly new notation. Zeta does not have an equivalence like tau so it is just a place holder.}

\begin{defn}
    The \textbf{edge attribute transfer function} transfers attributes of the hypergraph edges to the vertices of the $s$-line graph as $f_v: Y \to A$ such that $\epsilon(e_i) = \tau(e_i)$.
\end{defn}

\begin{defn}
    The \textbf{vertex attribute transfer function} transfers attributes of the hypergraph... \adm{Does it make sense to even have an attribute transfer function to the line graph edges?}
\end{defn}

If $f: \epsilon \to \tau$ \evg{is this a function in the usual sense?} is transferring edge attributes, we transfer attributes on the hyperedges $E$ in the hypergraph $H$ to the nodes $E$ of the line graph. For example, in our toy example, we transfer the interval hyperedge attributes and the edge marginalized topic attributes to the nodes of $\mathcal{L}_s$.
For transferring node attributes as $f: \phi \to \tau$, we can not directly transfer to the attribute line graph due to there being no direct representation of $V$ in $\mathcal{L}_s(H)$. As such, if there are node attributes either the clique expansion should be used in substitute of the line graph or an extension association should be performed to bring the node attributes to the incidences.
For an incidence attribute transfer function $f: \gamma \to \tau$ we transfer the incidence attributes for a hyperedge as a hash map data structure (also known as a dictionary) that captures the incidence relations for that hyperedge. For example, in Fig.~\ref{fig:topic_attributes}, if transferring the incidence topic attributes, we would transfer the hash map $\{ P_4: (A, B), P_5: (A, C) \}$ to node $M_1 \in \mathcal{L}_s(H)$.

Attributes can also be transferred to the line graph edges $f: H \to \zeta(K)$ to transfer information about hypergraph intersections. For example, these attributes could be as simple as the shared hyperedge vertices or the shared topics between hyperedges as in our toy example.

To generate the attribute line graphs in practice, we modified algorithm~2 of \cite{liu2022high} that uses hash maps to efficiently calculate $\mathcal{L}_s(H)$ as follows:
ALGORTHM


\begin{algorithm}
\caption{Algorithm to construct the attributed $s$-line graph $\mathcal{L}_s(H)$ for an attributed hypergraph $H$.}\label{alg:attributed_line_graph}
\begin{algorithmic}
\State $\mathcal{L}_s(H) \gets \emptyset$
\State $X \gets x$
\State $N \gets n$
\While{$N \neq 0$}
\If{$N$ is even}
    \State $X \gets X \times X$
    \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
\ElsIf{$N$ is odd}
    \State $y \gets y \times X$
    \State $N \gets N - 1$
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}



%\subsection{connection to s-walks}

Consider $H = (V,E)$ with attribute transferring function $f: H \to L_f(H)$ \evg{who is $L_f(H)$? } where $\tau_f(e) = \{v|vIe\}$. It is worth explicitly stating that the target \evg{range?} of $\tau_f$ is $2^V$. If we establish relation $S$ on elements of $2^V$ where for $a,b \in 2^V$ $aSb$ if $|a\cap b| \geq s$ then the s-walk graph is just the permissible walk graph on $L_f(H)$.
\begin{prop}
The s-walk graph of a hypergraph is the permissible walk graph on $L_f(H)$ for specific $f$.  
\end{prop}

\begin{defn}
Given vertex attributed graph $G = (V,E,\phi)$ where $\func{\phi}{V}{X}$ and relation $R$ on $X$ a \textbf{permissible walk on G} is a sequence of vertices $W = v_0v_1\ldots v_n$ where W is a walk in G and $\phi(W) = \phi(v_0)\phi(v_1)\ldots \phi(v_n)$ is a walk in $X$.
\end{defn}
\evg{is permissible walk definition necessary for permissible walk graph definition?}
\begin{defn}
Given attributed digraph $G = (V,E,\phi)$ with vertex attributions and a relation on those attributions $R$ a \textbf{permissible walk graph} is the directed subgraph \evg{subgraph of what?} $P(G) = (V,P(E))$ for which  $v_iP(E)v_j$  if $\phi(v_i)R\phi(v_j)$ and $v_iEv_j$. That is, two vertices in $P(G)$ are related if they are related by $E$ in $V$ and their attributions are related by $R$ in $X$.
\end{defn}

In this work we are interested in the specific case of the permissible walk graph of an attributed $s$-line graph.
\begin{defn} \label{def:permissible_s_line_graph}
Given attributed line graph $L(H) = (E,R, \tau, \zeta)$, the \textbf{permissible $s$-line graph} $L_p(H, s)$
is the directed subgraph $P(L) = (E,P(R))$ for which the $s$ condition, vertex relation, and edge relation are met.  The $s$-condition is the overlap of vertices as $e_i, e_j \in R$ $e_iP(R)e_j$ if $|a \cap b| \geq s$. The vertex relation is met with $e_iP(R)e_j$ if $\tau(e_i)L\tau(e_j)$, where $L$ is the required relation between vertices. The edge relation is met if $\zeta(r_i)$  is satisfied for $r_i \in R$.
\end{defn}
The $s$ condition can alternatively be considered as an edge relation with the attribute on the edges as $|a \cap b|$.





\subsection{Permissible Walk Graph} \label{ssec:permissible_walk_graph}

The permissible walk graph is constructed as a subgraph of the attributed $s$-line graph that respects the relations between attributes. 
We demonstrate the construction of permissible walk graphs using our toy example for how temporal intervals and set attributes can be used separately and combined.
\begin{defn} \label{def:permissible_walk_graph} \evg{haven't you already defined it in definition 7}
    We define the permissible walk graph $W_A = L_s \cap R_a$, where $R_a$ is our relation graph for the attribute $a$ in our set of attributes $A$. \evg{what is a relation graph $R_a$? }
\end{defn}
The relation graph for an attribute $a$ is created by checking if the relation is satisfied for all edges in the complete graph on the nodes in $\mathcal{L}_s$ using the attributes. \evg{this seems to be the definition of $R_a$. I still don't understand it, but either way it should come before the definition of $W_A$.} However, in practice, we only need to use the edges in $\mathcal{L}_s$ due to the intersection between graphs. For the toy example demonstration we show the relation graph for the complete graph to better show how these relations retrieve unique information.

To calculate $W_A(H,s)$ \evg{this notation differs from the one in definition} for an attributed $s$-line graph, we need to first define a relation on the attributes. In the context of of our toy example, which is a miniature meeting network represented as a hypergraph, we may be interested in capturing information on related meetings through their topics as well as the temporal ordering of meetings to understand which meeting influenced another. 
For the interval data we do this using the relation we define as the strong-inclusion ordering.
\begin{defn}
    The strong-inclusion relation\evg{in the previous paragraph you say ordering} between intervals sets a bi-directional edge if intervals have a non-empty overlap with $I_i \cap I_j \neq \emptyset$. If $I_i \cap I_j = \emptyset$, we set a directionality based on the strong order (i.e., from $I_i$ to $I_j$ if $I_i$ happens completely before $I_j$.
\end{defn}
Depending on the data source, there may be other relations that are more suitable, but based on the desire to capture information on the flow of meetings we chose to define this relation.

For the set attributes on edges we use the a comparable to the $s$-line graph, but on the projection of the hypergraph $H_S(V, S(E))$, where $S$ are the set attributes for the hyperedges $E$ that are also represented as hyperedges and $V$ is the vertex set. We set a bi-directional edge between nodes $e_i$ and $e_j$ in the relation graph $R_S(E, J)$ if $S(e_i) \cap S(e_j) \neq \emptyset$. \evg{I had a hard time parsing this paragraph, but ill give another try later.}

Returning to our toy example, the $s$-line graph for $s=1$ is shown in Fig.~\ref{fig:meeting_s_line_graph}, the interval relation graph $R_I$ using the strong-inclusion order is shown in Fig.~\ref{fig:meeting_temporal_respecting_graph}, and the topic relation graph $R_T$ is shown in Fig.~\ref{fig:meeting_relation_respecting_graph} with edges added if meetings share at least one topic using an edge marginalization function on the topics.

\begin{figure}[h] 
    \centering
    \begin{subfigure}[t]{.25\textwidth}
        \centering
        \includegraphics[width=.99\textwidth]{figures/meeting_s_line_graph.png}
        \caption{$L_s(H)$.}
        \label{fig:meeting_s_line_graph}
    \end{subfigure}
    \hspace{25pt}
    \begin{subfigure}[t]{.25\textwidth}
        \centering
        \includegraphics[width=.99\textwidth]{figures/meeting_temporal_respecting_graph.png}%
        \caption{$R_I$.}
        \label{fig:meeting_temporal_respecting_graph}
    \end{subfigure}
    \hspace{25pt}
    \begin{subfigure}[t]{.25\textwidth}
        \centering
        \includegraphics[width=.99\textwidth]{figures/meeting_relation_respecting_graph.png}%
        \caption{$R_T$.}
        \label{fig:meeting_relation_respecting_graph}
    \end{subfigure}
    \caption{The $s$-line graph $L_s$, temporal respecting graph $L_d$, and relation respecting graph $L_r$ for the toy example hypergraph in Fig.~\ref{fig:meeting_HG}.}
    \label{fig:meeting_HG_line_graphs}
\end{figure}

The line graph and two relation graphs in Fig.~\ref{fig:meeting_HG_line_graphs} capture information about the different attributes of the network. $L_s$ shows which meetings share $s\geq1$ participants capturing information about communication between people. The interval relation graph $R_I$ shows the chronological ordering of the meetings. Specifically, we can see that $M_1$ happens first with both $M_2$ and $M_3$ following and lastly $M_4$. This shows, for example, that $M_4$ could not have influenced the discussion in $M_1$.
Lastly, the topic set relation graph $R_T$ visualizes that $M_1$, $M_3$, and $M_4$ are all related, while $M_2$ is not based on the components since $M_2$ did not share any topics with the other meetings.

Our goal now is to create the permissible walks from the possible combinations of attributes using \label{def:permissible_walk_graph} to build different views of the network. 

While we do not show it, one could always consider the trivial case where we do not have any attributes and simply look at the $s$-line graph to capture information on the participant structure of the meetings. However, the goal of this work is to show how more information can be encoded into the permissible walk graph.
The first view shown in Fig.~\ref{fig:meeting_PW_graphs} is between the line graph and interval relation graph in Fig.~\ref{fig:meeting_PW_graph_temporal}. This graph captures information on the flow of meetings. Specifically, it shows that $M_1$ happened first with participants of that meeting splitting to go to $M_2$ and $M_3$ which happened concurrently. It also shows that participants from $M_3$ then went on to $M_4$. This shows that there could be influence from $M_1$ to $M_3$ and $M_2$ and a possibility of an influence from $M_1$ to $M_4$ (no guarantee of influence since $M_1$ and $M_4$ do not share an edge). However, this view does not capture information on the topics. 

\begin{figure}[h] 
    \centering
    \begin{subfigure}[t]{.25\textwidth}
        \centering
        \includegraphics[width=.99\textwidth]{figures/meeting_PW_graph_temporal.png}
        \caption{$W_I = L_s \cap R_I$.}
        \label{fig:meeting_PW_graph_temporal}
    \end{subfigure}
    \hspace{25pt}
    \begin{subfigure}[t]{.25\textwidth}
        \centering
        \includegraphics[width=.99\textwidth]{figures/meeting_PW_graph_relation.png}%
        \caption{$W_T = L_s \cap R_T$.}
        \label{fig:meeting_PW_graph_relation}
    \end{subfigure}
    \hspace{25pt}
    \begin{subfigure}[t]{.25\textwidth}
        \centering
        \includegraphics[width=.99\textwidth]{figures/meeting_PW_graph_relation_temporal.png}%
        \caption{$W_{I,T} = L_s \cap R_I \cap R_T$.}
        \label{fig:meeting_PW_graph_relation_temporal}
    \end{subfigure}
    \caption{The permissible walk graphs using the temporal information $W_t = L_s \cap R_I$, the relational information $W_r = L_s \cap R_T$, and the temporal and relational information $W_{I,T} = L_s \cap R_I \cap R_T$.}
    \label{fig:meeting_PW_graphs}
\end{figure}

We next investigate the example $W_T$ in Fig.~\ref{fig:meeting_PW_graph_relation}. Here we show that $M_1$, $M_3$ and $M_2$ are connected through both their participants and their topics with $M_2$ not being connected since it did not share any topics with the other meetings. This accurately captures the information that $M_1$ most likely did not influence $M_2$ as was the case in Fig.~\ref{fig:meeting_PW_graph_temporal} since they do not share any topics. However, $W_T$ does not capture temporal information and as such does not show that, for example, $M_3$ could not have influenced $M_1$ as is the case with $W_I$.

Our last  view is of the combined interval and topic attributes as $W_{I,T}$ in Fig.~\ref{fig:meeting_PW_graph_relation_temporal}. For this case we accurately capture all of the information. Namely, we show the temporal ordering of meetings using the interval information as well as the topic information with $M_2$ not being connected to $M_1$. While for this toy example the best option is to use both attributes as we were interested in which meetings influenced which, this is not always the case with the best attributes to include likely being based on the data analysis goal.

